Substochastic Monte Carlo Algorithms

In this paper we introduce and formalize Substochastic Monte Carlo (SSMC) algorithms. These algorithms, originally intended to be a better classical foil to quantum annealing than simulated annealing, prove to be worthy optimization algorithms in their own right. In SSMC, a population of walkers is initialized according to a known distribution on an arbitrary search space and varied into the solution of some optimization problem of interest. The first argument of this paper shows how an existing classical algorithm, "Go-With-The-Winners" (GWW), is a limiting case of SSMC when restricted to binary search and particular driving dynamics. Although limiting to GWW, SSMC is more general. We show that (1) GWW can be efficiently simulated within the SSMC framework, (2) SSMC can be exponentially faster than GWW, (3) by naturally incorporating structural information, SSMC can exponentially outperform the quantum algorithm that first inspired it, and (4) SSMC exhibits desirable search features in general spaces. Our approach combines ideas from genetic algorithms (GWW), theoretical probability (Fleming-Viot processes), and quantum computing. Not only do we demonstrate that SSMC is often more efficient than competing algorithms, but we also hope that our results connecting these disciplines will impact each independently. An implemented version of SSMC has previously enjoyed some success as a competitive optimization algorithm for Max-$k$-SAT.

==> a-v-figure1.tex <==
\begin{figure}[t]
    \begin{tikzpicture}[every node/.style={draw, circle, inner sep=0pt,minimum size=4pt},
    level distance=2em,
    level 1/.style={sibling distance=8em},
    level 2/.style={sibling distance=4em},
    level 3/.style={sibling distance=2em},
    level 4/.style={sibling distance=1em},
    level 5/.style={sibling distance=8em},
    level 6/.style={sibling distance=8em},
    level 7/.style={sibling distance=4em},
    level 8/.style={sibling distance=2em},
    level 9/.style={sibling distance=1em},
    level 10/.style={sibling distance=8em},
    level 11/.style={sibling distance=8em},
    level 12/.style={sibling distance=4em},
    level 13/.style={sibling distance=2em},
    level 14/.style={sibling distance=1em},
    level 15/.style={sibling distance=8em}
   ]
        \node {}
        child {node{}
            child{node{}
                child{node{}
                    child{node{}
                    }
                    child{node{}
                    }
                }
                child{node{}
                    child{node{}
                    }
                    child{node{}
                    }
                }
            }
            child{node{}
                child{node{}
                    child{node{}
                    }
                    child{node{}
                    }
                }
                child{node{}
                    child{node{}
                    }
                    child{node{}
                    }
                }
            }
        }
        child { node{}
        child { node{}
        child { node{}
        child { node{}
        child { node{}
            child { node{}
            child { node{}
            child { node{}
            child { node{}
            child { node{}
                    child {node{}
            child{node{}
                child{node{}
                    child{node{}
                    }
                    child{node{}
                    }
                }
                child{node{}
                    child{node{}
                    }
                    child{node{}
                    }
                }
            }
            child{node{}
                child{node{}
                    child{node{}
                    }
                    child{node{}
                    }
                }
                child{node{}
                    child{node{}
                    }
                    child{node{}
                    }
                }
            }
        }
        child { node{}
        child { node{}
        child { node{}
        child { node{}
        child { node{}
            child { node{} }
            child { node{} }
        }
        }
        }
        }
        }
            }
            }
            }
            }
            }
            child { node{}
                child{node{}
                   child{node{}
                        child{node{}
                        }
                        child{node{}
                        }
                    }
                    child{node{}
                        child{node{}
                        }
                        child{node{}
                        }
                    }
                }
                child{node{}
                    child{node{}
                        child{node{}
                        }
                        child{node{}
                        }
                    }
                    child{node{}
                        child{node{}
                        }
                        child{node{}
                        }
                    }
                }
            }
        }
        }
        }
        }
        };
    \end{tikzpicture}
\caption{Figure 1 of \cite{AV94}.}\label{fig:avfig1}
\end{figure}


==> proofs.tex <==
\section{Proofs}

\subsection{Proof of \Cref{lemma:compute}}\label{sec:proof-of-computational-lemma}
  
\begin{figure}[t]
\begin{center}
\begin{tikzpicture}
\draw[anchor=east] (-1,2) node {$V_{j-1}$};
\draw[anchor=east] (-1,1) node {$V_j$};
\draw[anchor=east] (-1,0) node {$V_{j+1}$};
\draw[very thin, dashed] (0,2) -- (0.5,1);
\draw[fill=white] (0,2) circle (0.05);
\draw[fill=black] (0.5,1) circle (0.05);
\draw (0.8,1) node {$x$};
\draw[very thin, dashed] (3,2) -- (3.5,1);
\draw[fill=white] (3,2) circle (0.05);
\draw[thick] (3.5,1) -- (3,0);
\draw (3,0.6) node {$w$};
\draw[fill=black] (3.5,1) circle (0.05);
\draw[fill=black] (3,0) circle (0.05);
\draw (3.8,1) node {$x$};
\draw (3.3,0) node {$y$};
\draw[very thin, dashed] (6,2) -- (6.5,1);
\draw[fill=white] (6,2) circle (0.05);
\draw[thick] (6.5,1) -- (6,0);
\draw[thick] (6.5,1) -- (7,0);
\draw[fill=black] (6.5,1) circle (0.05);
\draw[fill=black] (6,0) circle (0.05);
\draw[fill=black] (7,0) circle (0.05);
\draw (5.95,0.6) node {$w_1$};
\draw (7.05,0.6) node {$w_2$};
\draw (6.8,1) node {$x$};
\draw (6.3,0) node {$y$};
\draw (7.3,0) node {$z$};
\draw (8,1.5) node {$G_{j-1}$};
\draw (8,0.5) node {$G_j$};
\end{tikzpicture}
\end{center}
\caption{Three types of components in the subgraph $G_j$ in a binary tree.}\label{fig:graphs}
\end{figure}

  
    The subgraph $G_j$ decomposes into connected components of three types as to whether a node at depth $j$ is (i) a leaf, (ii) one child, or (iii) has multiple children at depth $j$. Note that nodes at layers $k < j$ are disconnected from subgraph $G_j$. See \cref{fig:graphs}.
  
    If either $x\in V_k$ for $k<j$ or $x\in V_j$ is a leaf, then the Laplacian component is just $L = 0$. The (relative) objective value is $(j-k+1)E$, and therefore the transition rate matrix is also $H = (j-k+1)E$. After time $t\in [0,1)$, we have
    \begin{equation}\label{eqn:ssmc-transition00}
        \mathrm{Pr}\{X(j+t) = x \:|\: X(j) = x\} =  e^{-(j-k+1)Et}.
    \end{equation}

    If $x\in V_j$ has a single child $y$ at depth $j+1$, and $w$ is the weight attached to the edge $(x,y)$, then our transition rate matrix on this component is
    \begin{equation*}
        H = \left(\begin{array}{cc} w & -w \\ -w & w\end{array}\right) + \left(\begin{array}{cc} E & 0 \\ 0 & 0\end{array}\right) = \begin{pmatrix} E + w & -w \\ -w & w\end{pmatrix}.
    \end{equation*}
    We can exponentiate this matrix in closed form to compute the transition probabilities at any time $t$, see \cref{sec:computations}, however since we are only interested in the limit of large $E$, we will work asymptotically in $\epsilon = \frac{w}{E}$. Diagonalizing the matrix $\tilde{H} = \frac{1}{E}H$ to order $\epsilon^3$ we have:
    \begin{equation*}
        \tilde{H}
        \begin{pmatrix} 1 & \epsilon \\ -\epsilon & 1 \end{pmatrix} =
        \begin{pmatrix} 1 & \epsilon \\ -\epsilon & 1 \end{pmatrix}
        \begin{pmatrix} 1 + \epsilon + \epsilon^2 & 0 \\ 0 & \epsilon - \epsilon^2 \end{pmatrix} + \bigO(\epsilon^3).
    \end{equation*}

    To derive the action of $e^{-Ht} = e^{-E\tilde{H}t}$ we compute
    $$
    e^{-Ht}\begin{pmatrix} 1 & \epsilon \\ -\epsilon & 1 \end{pmatrix} =
    \begin{pmatrix} 1 & \epsilon \\ -\epsilon & 1 \end{pmatrix}
    \begin{pmatrix} e^{-(E + w)t + \bigO(\epsilon)} & 0 \\ 0 & e^{-wt + \bigO(\epsilon)} \end{pmatrix} + \bigO(\epsilon^2).
    $$
    Notice that
    $$
    \begin{pmatrix} 1 & \epsilon \\ -\epsilon & 1 \end{pmatrix}
    \begin{pmatrix} 1 \\ \epsilon \end{pmatrix} = \begin{pmatrix} 1 \\ 0 \end{pmatrix} + \bigO(\epsilon^2).
    $$
    And so
    \begin{align*}
        e^{-Ht}\begin{pmatrix} 1 \\ 0 \end{pmatrix} &= \begin{pmatrix} 1 & \epsilon \\ -\epsilon & 1 \end{pmatrix} \begin{pmatrix} e^{-(E + w)t + \bigO(\epsilon)} \\ \epsilon e^{-wt + \bigO(\epsilon)} \end{pmatrix} + \bigO(\epsilon^2)\\
        &=\begin{pmatrix} e^{-(E + w)t + \bigO(\epsilon)} \\ \epsilon (e^{-wt + \bigO(\epsilon)} - e^{-(E + w)t + \bigO(\epsilon)})\end{pmatrix} + \bigO(\epsilon^2)
    \end{align*}
    That is,
    \begin{align}
       \Pr{X(j+t) = x \:|\: X(j) = x} &= e^{-(E+w)t + \bigO(1/E)} + \bigO(\tfrac{1}{E^2}),\label{eqn:transition10}\\
       \Pr{X(j+t) = y \:|\: X(j) = x} &= \frac{w}{E}e^{-wt} + \bigO(\tfrac{1}{E^2}).\label{eqn:transition11}
    \end{align}

    For a node $x\in V_j$ with $d$ children, $y_1, \dots, y_d \in V_{j+1}$, and associated edge weights $w_1, \dots, w_d$, the transition rate matrix is given by
    \begin{equation*}
       H = \begin{pmatrix} 
        E + w_1 + \cdots + w_d & -w_1 & \cdots & -w_d \\
       -w_1 & w_1 & \cdots & 0 \\
       \vdots & & \ddots \\
       -w_d & 0 & \cdots & w_d\end{pmatrix}
    \end{equation*}
    We introduce the notation $b_1 = \sum_{j=1}^d w_j$ and $b_2 = \sum_{j=1}^d w_j^2$.
    
    Let
    \begin{align*}
        \lambda_0 &= 1 + \frac{b_1}{E} + \frac{b_2}{E^2} + \bigO(\tfrac{1}{E^3})\\
       v_0 &= \begin{pmatrix} 1 \\ -\frac{w_1}{E} + \frac{w_1(b_1 - w_1)}{E^2}) \\ \vdots \\ -\frac{w_d}{E} +  \frac{w_d(b_1-w_d)}{E^2})\end{pmatrix} + \bigO(\tfrac{1}{E^3}).
    \end{align*}
    Then a direct computation shows both $\frac{1}{E}Hv_0$ and $\lambda_0v_0$ equal
    \begin{equation*}
        \begin{pmatrix} 1 \\ 0 \\ \vdots \\ 0 \end{pmatrix} + \frac{1}{E}\begin{pmatrix} b_1 \\ -w_1\\ \vdots \\ -w_d\end{pmatrix} + \frac{1}{E^2}\begin{pmatrix} b_2 \\ -w_1^2 \\ \vdots \\ -w_d^2\end{pmatrix} + \bigO(\tfrac{1}{E^3})
    \end{equation*}
    and so $Hv_0 = E\lambda_0v_0 + \bigO(\frac{1}{E^2})$.

    Let us assume for the moment that all the edge weights are distinct. Then for each $j=1, \dots, d$ define
    \begin{align*}
        \lambda_j &= \frac{w_j}{E} - \frac{w_j^2}{E^2} + \bigO(\tfrac{1}{E^3})\\
        v_j &= \begin{pmatrix} \frac{w_j}{E} + \frac{w_j^2}{E^2}\sum_{k\not=j} \frac{w_k}{w_j-w_k} \\ -\frac{1}{E}\frac{w_jw_1}{w_j-w_1} \\ \vdots \\ 1 \\ \vdots \\ -\frac{1}{E}\frac{w_jw_d}{w_j-w_d}\end{pmatrix} + \bigO(\tfrac{1}{E^3})
    \end{align*}
    Then a similar computation shows both $\frac{1}{E}Hv_j$ and $\lambda_jv_j$ equal
    \begin{equation*}
        \frac{1}{E}\begin{pmatrix} 0 \\ 0\\ \vdots \\ w_j \\ \vdots \\ 0\end{pmatrix} + \frac{1}{E^2}\begin{pmatrix} w_j^2 \\ -w_j^2w_1/(w_j-w_1) \\ \vdots \\ -w_j^2 \\ \vdots \\ -w_j^2w_d/(w_j-w_d)\end{pmatrix} + \bigO(\tfrac{1}{E^3})
    \end{equation*}
    and so $Hv_j = E\lambda_jv_j + \bigO(\frac{1}{E^2})$.

    Exponentiation, as in the proof of \cref{lemma:compute}, gives
    \begin{align*}
        e^{-Ht}v_0 &= e^{-(E + b_1)t + \bigO(1/E)}v_0 +\bigO(\tfrac{1}{E^2}),\\
        e^{-Ht}v_j &= e^{-w_jt + \bigO(1/E)}v_j + \bigO(\tfrac{1}{E^2})\text{ for $j=1, \dots, d$.}
    \end{align*}
    We also see
    \begin{equation*}
        \begin{pmatrix} 1 \\ 0 \\ \vdots \\ 0\end{pmatrix} = v_0 + \frac{w_1}{E}v_1 + \cdots \frac{w_d}{E}v_d + \bigO(\tfrac{1}{E^2}),
    \end{equation*}
    and therefore
    \begin{align*}
        e^{-Ht} \begin{pmatrix} 1 \\ 0 \\ \vdots \\ 0\end{pmatrix} &= e^{-(E + b_1)t +\bigO(1/E)}v_0 + \sum_{j=1}^d \frac{w_1}{E}e^{-w_jt +\bigO(1/E)} v_j + \bigO(\tfrac{1}{E^2})\\
        &= \frac{1}{E}\begin{pmatrix} 0 \\  w_1e^{-w_1t +\bigO(1/E)} \\ \vdots \\ w_de^{-w_dt +\bigO(1/E)} \end{pmatrix} + \bigO(\tfrac{1}{E^2}).
    \end{align*}
    Expressing this in terms of transition probabilities has
    \begin{align*}
        \Pr{X(j+t) = x \:|\: X(j) = x} &= \bigO\left(\tfrac{1}{E^2}\right),\\
        \Pr{X(j+t) = y_j \:|\: X(j) = x} &= \frac{w_j}{E}e^{-w_jt} + \bigO\left(\frac{1}{E}\right),
    \end{align*}
    for each $j=1, \dots, d$.

    Note that the resulting transition probabilities vary smoothly with small perturbations in the weights $w_j$. Therefore if not all the weights are distinct, one perturbs them slightly into distinct values, and the above analysis produces the desired expression.

\subsection{Proof of \Cref{thm:limit-process}}\label{sec:proof-of-limit-theorem}

    Initially, we have $\Pr{X_E(0) = \text{root}} = \Pr{X(0) = \text{root}} = 1$ and so $\delta(X_E(0),X(0)) = 0$. Inductively, assume that at time $t = j$ we $\delta(X_E(j),X(j)) =\bigO(\frac{1}{E})$. 
    
    We first compute the normalization term $\Pr{X_E(j+1) \not= \infty \:|\: X_E(j)\not=\infty}$. In general this is
    \begin{align*}
        &\Pr{X_E(j+1) \not=\infty\:|\: X_E(j)\not=\infty}\\
        &\quad = \sum_{x\in G} \Pr{X_E(j+1) \not=\infty\:|\:X_E(j) = x}\Pr{X_E(j) = x\:|\: X_E(j)\not=\infty}\\
        &\quad = \sum_{x,y\in G} \Pr{X_E(j+1) =y\:|\:X_E(j) = x}\Pr{X_E(j) = x\:|\: X_E(j)\not=\infty}.
    \end{align*}
    Note that by \cref{lemma:compute}, $\Pr{X_E(j+1) =y\:|\:X_E(j) = x}$ is negligible in $E$ unless $x,y \in G_j$. Even then, $\Pr{X_E(j+1) =y\:|\:X_E(j) = x} =\bigO(\frac{1}{E^2})$ unless $y$ is a child of $x$. So, given $x\in V_j$ with child $y\in V_{j+1}$ \Cref{lemma:compute} gives
    \begin{equation*}
        \Pr{X_E(j+1) =y\:|\:X_E(j) = x} = \frac{w_{xy}}{E}e^{-w_{xy}} +\bigO(\tfrac{1}{E^2}).
    \end{equation*}
    Therefore, since $\delta(X_E(j),X(j)) =\bigO(\frac{1}{E})$ by hypothesis
    \begin{align*}
        &\Pr{X_E(j+1) \not=\infty\:|\: X_E(j+1)\not=\infty}\\
        &\quad = \sum_{y\in V_{j+1}}\sum_{x\in V_j} \frac{a_{xy}}{E} \Pr{X_E(j) = x\:|\: X_E(j) \not=\infty} +\bigO(\tfrac{1}{E^2})\\
        &\quad = \sum_{y\in V_{j+1}}\sum_{x\in V_j} \frac{a_{xy}}{E} \Pr{X(j) = x} +\bigO(\tfrac{1}{E^2}).
    \end{align*}
    
    Now for a general $y\in V_{j+1}$ with parent $x\in V_j$, again using \Cref{lemma:compute} and the inductive hypothesis,
    \begin{align*}
        &\Pr{X_E(j+1) = y\:|\: X_E(j+1)\not=\infty}\\
        &\quad = \frac{\Pr{X_E(j+1) = y\:|\:X_E(j) = x}\Pr{X_E(j) = x\:|\: X_E(j)\not=\infty}}{\Pr{X_E(j+1) \not= \infty \:|\: X_E(j)\not=\infty}}\\
        &\quad = \frac{\left(\frac{a_{xy}}{E} +\bigO(\frac{1}{E^2})\right)\left(\Pr{X(j) = x} +\bigO(\frac{1}{E})\right)}{\sum_{y'\in V_{j+1}}\sum_{x'\in V_j} \frac{a_{x'y'}}{E} \Pr{X(j) = x'} +\bigO(\tfrac{1}{E^2})}\\
        &\quad = \frac{\sum_{x\in V_j} a_{xy}\Pr{X(j) = x}}{\sum_{y'\in V_{j+1}}\sum_{x'\in V_j} a_{x'y'}\Pr{X(j) = x'}} +\bigO(\tfrac{1}{E})\\
        &\quad = \Pr{X(j+1) = y} +\bigO(\tfrac{1}{E}).
    \end{align*}
    Therefore $\delta(X_E(j+1),X(j+1)) =\bigO(\frac{1}{E})$.
    

\subsection{Proof of \Cref{thm:comb}}\label{sec:comb}

    To compute the probability that \cref{alg:GWW1*} succeeds at reaching the deepest node of the comb tree (\cref{fig:comb}), we begin by supposing that we have a total population of $N$ walkers. Let $Y_j$ be the node on the left hand tooth at depth $j$. Because \cref{alg:GWW1*} always has $\eta_k(Y_j) = \eta_j(Y_j)\delta_{jk}$, we let $\eta(Y_j) = \eta_j(Y_j)$. We wish to derive a bound for \( P(\eta(Y_{d-1}) = N) \). 
    
    First, note that for $j < d$, $P(\eta(Y_{j+1}) < \eta(Y_j)) = 0$. That is, because \cref{alg:GWW1*} has all walkers on the left tooth continue to child nodes, there is no probability that any walker will jump to the spine unless $j=d$. 
    
    Where we do not not expect that it will cause confusion, we abusively write $\eta(v)$ for the set of walkers at a particular vertex, as well as the number of walkers at that vertex. Consider, now, the population $\eta(b_j)$ of walkers on the right hand branch $b_j$ at depth $j$. Note that each walker $w\in \eta(b_j)$ has a probability of $1/2$ of advancing to either of the right hand nodes at depth $j+1$. Denote by $l_j$ the leaf at depth $j$. After the walkers move, then probability that each walker at the leaf moves to the left hand branch is given by 
    \[
        \Pr{w \in \eta(b_{j+1}) | w \in \eta(b_j)} = \frac{\eta(Y_j)}{N-\eta(l_{j+1})} \geq \frac{\eta(Y_j)}{N}.
    \]
    Now, we find that
    \begin{align*}
        \Pr{w \in \eta(b_{j+1}) | w \in \eta(b_j)} &=1-\Pr{w \in \eta(b_{j+1}) | w \in \eta(l_{j+1})}\Pr{w \in \eta(l_{j+1}) \vert w \in \eta(b_j)} \\
        &\leq \left(1-\frac{\eta(Y_j)}{2 N}\right).
    \end{align*}
    Thus, the probability that a walker at depth $0$ is in $\eta(b_{j+1})$ is given by,
    \begin{align*}
        \Pr{w \in \eta(b_{j+1}) \vert w \in \eta(b_0)} &= \prod_{k=0}^{j} \Pr{w \in \eta(b_{k+1}) \vert w \in \eta(b_k)}  \\
        &\leq \prod_{k=1}^{j} \left(1-\frac{\eta(Y_j)}{2 N}\right) \\
        &\leq \left(1-\frac{\eta(Y_1))}{2 N}\right)^{j}\\
        &\leq \exp\left(-\frac{\eta(Y_1)}{2 N} j \right).
    \end{align*}
    Thus, 
    \begin{align*}
        \Pr{\eta(b_0) \subseteq \eta(Y_{j+1})} &\geq \left(1- \exp\left(-\frac{\eta(Y_1)}{2 N} j \right)\right)^{N-\eta(Y_1)} \\
        &\geq 1-\left(N-\eta(Y_1)\right)\exp\left(-\frac{\eta(Y_1)}{2 N} j \right).
    \end{align*}
    Hence, 
    \begin{equation}\label{eqn:store}
        \Pr{\eta(b_0) \subset \eta(Y_{j+1}) \vert \eta(Y_1) \geq y } \geq 1-(N-y)\exp\left(-\frac{y}{2 N} j \right).
    \end{equation}
    \begin{align*}
        \Pr{\eta(b_0) \subset \eta(Y_{j+1})} &\geq \sup_\delta \left(
            \Pr{\eta(b_0) \subset \eta(Y_{j+1}) \vert \eta(Y_1) \geq \frac{N}{2}-\delta}\Pr{\eta(Y_1) \geq \frac{N}{2} - \delta} \right)\\
            &\geq \sup_\delta \left(\Pr{\eta(b_0) \subset \eta(Y_{j+1}) \vert \eta(Y_1) \geq \frac{N}{2} - \delta} \left(1-e^{-2 \frac{\delta^2}{N}} \right)\right)\\
            &\geq \sup_\delta \left( 1-\left(\frac{N}{2}+\delta\right)\exp\left(-(1/4-\frac{\delta}{2N}) j \right)\right)\left(1-e^{-2 \frac{\delta^2}{N}} \right)
    \end{align*}
    where we have used Hoeffding's inequality and \cref{eqn:store}. For simplicity, take $\delta = c_1\frac{N}{2}$. Then, we have that
    \[
         \Pr{\eta(b_0) \subset \eta(Y_{j+1})} \geq (1-(1+c_1)\frac{N}{2}e^{-(1-c_1)\frac{j}{4}})(1-e^{-\frac{c_1^2 N}{4}}) = 1 -\bigO(Ne^{-j}) -\bigO(e^{-N})
    \]
    so that the probability that all walkers end on the left branch approaches 1 exponentially quickly in both depth and total number of walkers.
    
    Now, if the depth of the tree is $d+1$ and the depth of the left hand side is $j$, we have that 
    \begin{align*}
        \Pr{\eta(b_{d+1}) \neq \emptyset} &= \Pr{\eta(b_d) \neq \emptyset}\\
        &\leq 1 - \Pr{\eta(b_0) \subset \eta(Y_{j+1})}\\
        &\leq \mathcal{O}(N e^{-j}) + \mathcal{O}(e^{-N}).
    \end{align*}

\subsection{Proof of \Cref{thm:waterfall2}}\label{sec:waterfall2}\newcommand{\half}{\frac{1}{2}}
        Suppose that $b_i$ is the branch at level $i$. Then, let $B \subseteq V_{i+1}$ be the children of $b_i$. Note that no walkers at $b_i$ stay behind. Also, note that $m_{i+\half}(V_i) < 1$ by the construction of the algorithm. 
        \begin{align}
            \E{m_{i+1}(b_{i+1})\vert m_i(b_i)} &= \frac{1}{2}\E{m_{i+1}(B)\vert m_i(b_i)} \nonumber \\
            &= \frac{1}{2}\E{m_i(b_i) + m_i(b_i)\frac{m_{i+\half}(V_i)}{1-m_{i+\half}(V_i)} \vert m_i(b_i)} \nonumber\\
            &=\frac{m_i(b_i)}{2}\left(1+\E{\frac{m_{i+\half}(V_i)}{1-m_{i+\half}(V_i)} \vert m_i(b_i) }\right) \nonumber\\
            &\geq \frac{m_i(b_i)}{2}\left(1+\frac{\E{m_{i+\half}(V_i) \vert m_i(b_i)}}{1-\E{m_{i+\half}(V_i) \vert m_i(b_i)} }\right) \nonumber\\
            &= \frac{m_i(b_i)}{2}\left(1+\frac{\frac{1 - m_i(b_i)}{2}}{1-\frac{1 - m_i(b_i)}{2} }\right) \nonumber\\
            &=  \frac{m_i(b_i)}{1 + m_i(b_i)} \nonumber
        \end{align}
        where we have used the fact that the two vertices in $B$ have equal expected values and Jensen's inequality. To bound the decay rate, we define the new statistic, $\overline{m}_i = \min(m_i(b_i),\frac{1}{i+1})$. Note that $\overline{m}_i \leq m_i(b_i)$ and so conditioning on when this inequality is strict gives
        \begin{align*}
            \E{\overline{m}_{i+1}} &\geq \E{\frac{m_i(b_i)}{1 + m_i(b_i)} \vert m_i(b_i) 
            = \overline{m}_i}\Pr{m_i(b_i) 
            = \overline{m}_i} + \frac{1}{i+2}\Pr{m_i(b_i) 
            > \overline{m}_i} \\
            &= \E{\frac{\overline{m}_i}{1+\overline{m}_i}}\\
            &\geq \left(\frac{1+i}{2+i}\right)\E{\overline{m}_i}
        \end{align*}
        where the first inequality follows from the monotonicity of $\frac{u}{1+u}$ and the second inequality from increasing the denominator to its largest possible value.
        
        Solving the recurrence in $E(\overline{m}_i)$ yields
        \[
            \E{m_i(b_i)} \geq \E{\overline{m}_i} \geq \frac{1}{i+1}.
        \]        
        Now, we can apply Markov's inequality,
        \begin{align*}
            \Pr{m_{i}(b_i) \geq \frac{1}{N}} &\geq 1-\frac{1-\E{m_{i}(b_i)}}{1-\frac{1}{N}} \\
            &= 1-\frac{N-\frac{N}{i+1}}{N-1}
        \end{align*}
        and for $N \geq i$ we have the desired result,
        \[
            \Pr{m_{i}(b_i) \geq 1} \geq \frac{1}{i}-\frac{1}{N}.
        \]

    \subsection{Sketch of proof of \cref{prop:descent}}\label{proof:propdescent}
        We prove this in the case that all walkers are initialized to the same site $u$ and then sketch the proof for other distributions. Suppose that, initially, all walkers occupy vertex $u$. Then, $\Delta E = 0$. Thus, by \cref{eqn:grad}, no walkers transition to $\infty$. Now, let $T_{u\mapsto v} \leq 1 - T_{u\mapsto v}$ be the probability that walkers transition to site $v$, with $W(v) < W(u)$. Then, the probability that at least one walker jumped to state $v$ is given by
        \[
            \Pr{m_{t+1}(v) \neq 0} \geq 1 - (1 - T_{u\mapsto v})^N.
        \]
        Now, all walkers are distributed between two sites, where we have $T_{\xi_i \mapsto \infty} = \frac{\Delta E}{(1-t)+t \Delta E}$. Thus, 
        \[
            \Pr{m_{t+1+\half}(v) = 0 } \geq \left(\frac{\Delta E}{(1-t)+t \Delta E}\right)^N.
        \]
        Hence, 
        \begin{align*}
            \Pr{m_{t+2}(v) = N} &\geq \left(1 - (1 - T_{u\mapsto v})^N\right)\left(\frac{t \Delta E}{(1-t)+t \Delta E}\right)^N \\
            &\geq (1-e^{-N T_{u\mapsto v}})e^{-N\frac{1-t}{t \Delta E}}\\
            &\geq (1-e^{-N T_{u\mapsto v}})(1-N\frac{1-t}{t \Delta E})
        \end{align*}        
    
    To prove \cref{prop:descent} in full generality, one only needs to consider the behavior of the tail of the walkers occupying the highest site in the distribution. The proof simplifies, because the only behavior that needs to be considered up to $\bigO(\frac{N}{\Delta E})$ is the jump process. 

\endinput

    If our node $x$ has two children, $y$ and $z$, at depth $j$ with edge weights $w_1$ and $w_2$ for transitions from $x$ to $y$ and $z$ respectively, we have the transition rate matrix
    \begin{equation*}
        H = \left(\begin{array}{ccc} E+w_1+w_2 & -w_1 & -w_2\\ -w_1 & w_1 & 0\\-w_2 & 0 & w_2\end{array}\right).
    \end{equation*}
    As above we set $\epsilon = w_1/E$ and write $c = \frac{w_2}{w_1}$. Then
    \begin{equation*}
        \tilde{H} = \tfrac{1}{E} H = \begin{pmatrix}1 + (c+1)\epsilon & -\epsilon & -c\epsilon \\ -\epsilon & \epsilon & 0\\ \ -c\epsilon & 0 & c\epsilon \end{pmatrix}.
    \end{equation*}
    There are two distinct analyses according to whether $c=1$ or $c\not=1$.

    In case $c = 1$, that is $w_1 = w_2 = w$, we have $\tilde{H} V = V \Lambda +\bigO(\epsilon^3)$ where
    \begin{align*}
       V &= \begin{pmatrix} 1 & 2\epsilon & 0 \\ -\epsilon + \epsilon^2 & 1 + \epsilon & 1\\ -\epsilon + \epsilon^2 & 1 + \epsilon & -1\end{pmatrix}\\
       \Lambda &= \begin{pmatrix} 1 + 2\epsilon + 2\epsilon^2 & 0 & 0\\ 0 & \epsilon - 2\epsilon^2 & 0\\ 0 & 0 & \epsilon \end{pmatrix}.
    \end{align*}
    So
    \begin{equation*}
        e^{-Ht}V = V\begin{pmatrix} e^{-(E + 2w)t +\bigO(\epsilon)} & 0 & 0\\ 0 & e^{-wt +\bigO(\epsilon)} & 0\\ 0 & 0 & e^{-wt +\bigO(\epsilon)} \end{pmatrix} +\bigO(\epsilon^2).
    \end{equation*}
    Now,
    \begin{equation*}
        \begin{pmatrix} 1 & 2\epsilon & 0 \\ -\epsilon & 1 + \epsilon & 1\\ -\epsilon & 1 + \epsilon & -1\end{pmatrix}\begin{pmatrix} 1 \\ \epsilon\\ 0\end{pmatrix} =  \begin{pmatrix} 1 \\ 0 \\ 0\end{pmatrix} +\bigO(\epsilon^2)
    \end{equation*}
    and we find
    \begin{align*}
       e^{-Ht}\begin{pmatrix} 1 \\ 0 \\ 0\end{pmatrix} 
        &= \begin{pmatrix} 1 & 2\epsilon & 0 \\ -\epsilon & 1 + \epsilon & 1\\ -\epsilon & 1 + \epsilon & -1\end{pmatrix}\begin{pmatrix} e^{-(E+2w)t+O(\epsilon)}\\ e^{-wt+O(\epsilon)}\\ 0 \end{pmatrix} +\bigO(\epsilon^2)\\
       &= 
       \begin{pmatrix}
            e^{-(E+2w)t+O(\epsilon))}\\
           \epsilon\left(e^{-wt+O(\epsilon)} - e^{-(E+2w)t+O(\epsilon)}\right)\\
           \epsilon\left(e^{-wt+O(\epsilon)} - e^{-(E+2w)t+O(\epsilon)}\right)
       \end{pmatrix} +\bigO(\epsilon^2).
    \end{align*}
    In terms of transition probabilities, this is
    \begin{align}
       \Pr{X(j+t) = x \:|\: X(j) = x} &= e^{-(E+2w)t+O(1/E))} +\bigO(\tfrac{1}{E^2})\label{eqn:transition20}\\
       \Pr{X(j+t) = y_1 \:|\: X(j) = x} &= \frac{w}{E}\left(e^{-wt+O(1/E)} - e^{-(E+2w)t+O(1/E)}\right) +\bigO(\tfrac{1}{E^2})\label{eqn:transition21}\\
       \Pr{X(j+t) = y_2 \:|\: X(j) = x} &= \frac{w}{E}\left(e^{-wt+O(1/E)} - e^{-(E+2w)t+O(1/E)}\right) +\bigO(\tfrac{1}{E^2}).\label{eqn:transition22}
    \end{align}

    Finally we treat the case $c\not= 1$. One can easily verify $\tilde{H} V = V \Lambda +\bigO(\epsilon^3)$ where
    \begin{align*}
        V &= \begin{pmatrix} 1 & (c-1)\epsilon + c\epsilon^2 & c(c-1)\epsilon - c^2\epsilon^2\\ -\epsilon + c\epsilon^2 & c-1 & -c\epsilon\\ -c\epsilon + c\epsilon^2  & c\epsilon & c-1 \end{pmatrix}\\
        \Lambda &= \begin{pmatrix} 1 + (c+1)\epsilon + (c^2+1)\epsilon^2 & 0 & 0\\ 0 & \epsilon - \epsilon^2 & 0\\ 0 & 0 & c\epsilon - c^2\epsilon^2 \end{pmatrix}.
    \end{align*}
    So
    \begin{align*}
       e^{-Ht}V = V \begin{pmatrix} e^{-(E+w_1+w_2)t+O(\epsilon)} & 0 & 0\\ 0 & e^{-w_1t+O(\epsilon)} & 0\\ \ 0 & 0 & e^{-w_2t+O(\epsilon)} \end{pmatrix} +\bigO(\epsilon^2).
    \end{align*}
    We have
    \begin{equation*}
        V\begin{pmatrix} 1 \\ \tfrac{1}{c-1}\epsilon\\ \tfrac{c}{c-1}\epsilon\end{pmatrix} =  \begin{pmatrix} 1 \\ 0 \\ 0\end{pmatrix} +\bigO(\epsilon^2)
    \end{equation*}
    and so
    \begin{align*}
        e^{-Ht}\begin{pmatrix} 1 \\ 0 \\ 0\end{pmatrix} 
        &= \begin{pmatrix} 1 & (c-1)\epsilon& c(c-1)\epsilon\\ -\epsilon & c-1 & -c\epsilon\\ -c\epsilon & c\epsilon & c-1 \end{pmatrix}\begin{pmatrix} e^{-(E+w_1+w_2)t+O(\epsilon)}\\ \tfrac{\epsilon}{c-1}e^{-w_1t+O(\epsilon)}\\ \tfrac{c\epsilon}{c-1}e^{-w_2t+O(\epsilon)} \end{pmatrix} +\bigO(\epsilon^2)\\
        &= 
        \begin{pmatrix}
            e^{-(E+w_1+w_2)t+O(\epsilon))}\\
            \epsilon\left(e^{-w_1t+O(\epsilon)} - e^{-(E+w_1+w_2)t+O(\epsilon)}\right)\\
            c\epsilon\left(e^{-w_2t+O(\epsilon)} - e^{-(E+w_1+w_2)t+O(\epsilon)}\right)
        \end{pmatrix} +\bigO(\epsilon^2).
    \end{align*}
    That is,
    \begin{align*}
        \Pr{X(j+t) = x \:|\: X(j) = x} &= e^{-(E+w_1+w_2)t+O(1/E))} + \bigO(\tfrac{1}{E^2})\\
        \Pr{X(j+t) = y_1 \:|\: X(j) = x} &= \frac{w_1}{E}\left(e^{-w_1t+O(1/E)} - e^{-(E+w_1+w_2)t+O(1/E)}\right) + \bigO(\tfrac{1}{E^2})\\
        \Pr{X(j+t) = y_2 \:|\: X(j) = x} &= \frac{w_2}{E}\left(e^{-w_2t+O(1/E)} - e^{-(E+w_1+w_2)t+O(1/E)}\right) + \bigO(\tfrac{1}{E^2}).
    \end{align*}
    In particular, we see that while the method of analysis when $c\not= 1$ differs, the transition probability have the same rule as when $c = 1$, \cref{eqn:transition20,eqn:transition21,eqn:transition22}.



==> waterfall.tex <==
\begin{figure}[ht]\centering
    \begin{tikzpicture}[every node/.style={draw, circle, inner sep=0pt,minimum size=4pt},
    level/.style={sibling distance=7em}
    ]
        \node {}
        child {node {}
                child { node {}
                    child { node {}
                        child { node {} edge from parent[dotted] 
                            %child { node[solid] {} edge from parent[solid]
                                %child { node[solid] {} edge from parent[dotted]}
                            %}
                        }
                    }
                }
            }
        child {node {}
                child {node {}
                    child { node {}
                        child { node {} edge from parent[dotted] 
                            %child { node[solid] {} edge from parent[solid]
                                %child { node[solid] {} edge from parent[dotted]}
                            %}
                        }
                    }
                }
                child{ node {} 
                    child{ node {} 
                            child { node {} edge from
                                parent[dotted]
                                    %child { node[solid] {} edge from parent[solid]
                                        %child { node[solid] {} edge from parent[dotted]}
                                    %}
                            }
                         }
                    child{ node {} edge from parent[dotted] {
                        child{ node [solid] {} edge from     parent[solid] 
                                %child { node[solid] {} edge from parent[solid] %child { node[solid] {} edge from parent[dotted]}
                            %}
                        }
                        child{ node [solid] {} edge from parent[solid] %child { node[solid] {} edge from         parent[solid] child { node[solid] {} edge from parent[solid]
                            %child { node[solid] {} edge from parent[solid]}            
                        }}%}}
                        }
                    }
            };
    \end{tikzpicture}
\caption{A comb tree with many long teeth.}\label{fig:waterfall}
\end{figure}
